Defect engineering in two-dimensional pentagonal PdTe$_2$: Tuning electronic, optical, and magnetic properties

Recently, the successful synthesis of the pentagonal form of PdTe$_{2}$ monolayer (\emph{p}-PdTe$_{2}$) was reported [Liu~\emph{et al.}, Nature Materials \textbf{23}, 1339 (2024)]. In this work, we present an extensive first-principles density-functional theory (DFT) based computational study of vacancies in this material. Our study covers the evolution of the electronic, optical, and magnetic properties of various defect configurations and compares those to the pristine monolayer (\emph{p}-PdTe$_{2}$). We find that V$_{Pd}$ (V$_{Te}$) is the most stable defect in the~\emph{p}-PdTe$_{2}$ monolayer in the Te-rich (Pd-rich) limit. The defects alter the electronic properties of the monolayer significantly, leading to changes in their magnetic and optical properties due to the emergence of midgap impurity states. The defect complex V$_{Pd+4Te}$ is found to induce spin-polarization in the system with a total magnetic moment of 1.87 $\mu_{B}$. The obtained low diffusion energy barriers of 1.13 eV (in-plane) and 0.063 eV (top-bottom) corresponding to V$_{Te}$ indicates its facile migration probability is higher in the top-bottom direction at room temperature, as revealed by AIMD simulations as well. In order to guide the experimentalists, we also simulated the scanning-tunneling microscope (STM) images corresponding to all the defect configurations. Moreover, we also computed the electron-beam energies required for creating mono-vacancies. In the optical absorption spectra of the defective configurations, finite peaks appear below the band edge that are unique to the respective defective configuration. We have also computed the excess polarizability of the defective configurations with respect to the pristine one and found that maximum changes occur in the infrared and visible regions, providing insights into the change in their optical response as compared to the pristine monolayer.

==> checklab.tex <==
 % Making those `Label(s) have changed\dots' messages more explicit
%
% The \LaTeX{} kernel produces the messages when something, while the
% |.aux| file is being scanned (after the \cs{AtEndDocument} tokens
% have been executed), sets the \cs{if@tempswa} switch with the
% command \cs{@tempswatrue}.
%
% (This fact can be used by packages, such as my |footmisc.sty|, to
% piggy-back on the message; but it's nice in that circumstance and
% others to be sure where the message is coming from.)
%
% This is a jiffy patch to the kernel so that it produces a
% (\cs{typeout}) message for each label \emph{it} thinks has changed.
%
% Usage: Incorporate this code into a package or class file,       or
%        \input this file from a package or class file,            or
%        \makeatletter \input{checklab} \makeatother in your document
%                                                    preamble
%
% This software jiffy is placed in the public domain.  Do with it as
% you wish, though I have to say I would prefer you not to claim it
% as your own (otoh, it's the product of a twisted mind, so probably
% not an attractive thing to claim).
%
% Robin Fairbairns (rf10@cl.cam.ac.uk)
% Produced in this form 1999/01/15
%
\def\@testdef #1#2#3{%
  \def\reserved@a{#3}%
  \expandafter \ifx \csname #1@#2\endcsname \reserved@a
  \else
    \@tempswatrue
    \typeout{label change: #1@#2 was
      \expandafter \ifx \csname #1@#2\endcsname \relax
        unset
      \else
        \csname#1@#2\endcsname\space
      \fi
      now #3}%
  \fi
}


==> removefr.tex <==
%Date: Sat, 30 Jul 1994 17:58:55 PST
%From: Donald Arseneau <asnd@erich.triumf.ca>
%
%  \@removefromreset{FOO}{BAR} : Removes counter FOO from the list of
%                       counters \cl@BAR to be reset when counter BAR
%                       is stepped.  The opposite of \@addtoreset.

\def\@removefromreset#1#2{\let\@tempb\@elt
   \expandafter\let\expandafter\@tempa\csname c@#1\endcsname
   \def\@elt##1{\expandafter\ifx\csname c@##1\endcsname\@tempa\else
         \noexpand\@elt{##1}\fi}%
   \expandafter\edef\csname cl@#2\endcsname{\csname cl@#2\endcsname}%
   \let\@elt\@tempb}

